Team HYU ASML ROBOVOX SP Cup 2024 System Description

This report describes the submission of HYU ASML team to the IEEE Signal Processing Cup 2024 (SP Cup 2024). This challenge, titled "ROBOVOX: Far-Field Speaker Recognition by a Mobile Robot," focuses on speaker recognition using a mobile robot in noisy and reverberant conditions. Our solution combines the result of deep residual neural networks and time-delay neural network-based speaker embedding models. These models were trained on a diverse dataset that includes French speech. To account for the challenging evaluation environment characterized by high noise, reverberation, and short speech conditions, we focused on data augmentation and training speech duration for the speaker embedding model. Our submission achieved second place on the SP Cup 2024 public leaderboard, with a detection cost function of 0.5245 and an equal error rate of 6.46%.

==> tables/table1.tex <==
\begin{table}[t] \begin{center}
%\captionsetup{singlelinecheck = false, justification=justified}
%\caption{FLOPs of SE extraction methods on the $30$-s audio signal, where + FT denotes the proposed extraction method with the fine-tuning SE model.}
%\caption{FLOPs of SE extraction methods on the $30$-s audio signal, where FT denotes the fine-tuned SE model.}
\caption{ResNet-100 architecture} 
\centering
\begin{tabular}{lcr}
\toprule
\textbf{Layer name} & \textbf{Structure} & \textbf{Output} \\ 
\midrule 
Conv2D & $3 \times 3$, 128, stride=1 & $\mathrm{128 \times 96 \times T}$  \\
\midrule
ResBlock-1 & $\begin{bmatrix}
    3 \times 3, 128 \\
    3 \times 3, 128 \\
    \mathrm{fwSE},[128, 96]
\end{bmatrix} \times 6$ & $\mathrm{128 \times 96 \times T}$  \\
\midrule
ResBlock-2 & $\begin{bmatrix}
    3 \times 3, 128 \\
    3 \times 3, 128 \\
    \mathrm{fwSE},[128, 48]
\end{bmatrix} \times 16$ & $\mathrm{128 \times 48 \times T/2}$ \\
\midrule
ResBlock-3 & $\begin{bmatrix}
    3 \times 3, 128 \\
    3 \times 3, 128 \\
    \mathrm{fwSE},[128, 24]
\end{bmatrix} \times 24$ & $\mathrm{256 \times 24 \times T/4}$ \\
\midrule
ResBlock-4 & $\begin{bmatrix}
    3 \times 3, 128 \\
    3 \times 3, 128 \\
    \mathrm{fwSE},[128, 12]
\end{bmatrix} \times 3$ & $\mathrm{256 \times 12 \times T/8}$ \\
\midrule
Flatten(C, F) & --- & $\mathrm{3072 \times T/8}$ \\
CAS & --- & 6144 \\
\midrule
Dense & --- & 256 \\
AM-Softmax & --- & Num. of speakers \\
\bottomrule 
\end{tabular}
\end{center}
\end{table}
%

==> tables/table2.tex <==
\begin{table}[t] \begin{center}
%\captionsetup{singlelinecheck = false, justification=justified}
%\caption{EER on two SV protocols, where FT denotes the fine-tuned SE model.}
\caption{EER on two SV protocols.}
\resizebox{0.95\columnwidth}{!}{
\begin{tabular} {ccccc}
\toprule

\multicolumn{1}{c}{\multirow{2}{*}{\textbf{SE Model}}}&
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}}&
\multicolumn{3}{c}{\textbf{SE Extraction Method}}\\
& & {Conventional} & {Proposed} & {Proposed+FT}  \\
\midrule
{\textbf{ECAPA-}}
& {VoxCeleb1-O}
& {1.35\%} & {2.09\%} & {1.66\%} \\
{\textbf{TDNN}}
& {VoxConverse}
& {16.04\%} & {17.54\%} & {15.97\%} \\
\midrule
{\textbf{Fast-}}
& {VoxCeleb1-O}
& {2.16\%} & {3.39\%} & {2.49\%} \\
{\textbf{ResNet}}
& {VoxConverse}
& {17.32\%} & {18.57\%} & {16.79\%} \\


%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{SE Model}}}&
%%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{SE Extraction Method}}}&
%{\textbf{SE Extraction}}&
%\multicolumn{3}{c}{\textbf{Datasets}}\\
%& {\textbf{Method}}& {VoxCeleb1-O} & {DIHARD III} & {VoxConverse}  \\
%%&& {0.5 s} & {1.0 s} & {1.5 s} & {2.0 s} \\
%\midrule
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ECAPA-}}}
%& {Conventional}
%& {1.35\%} & {00.00\%} & {00.00\%} \\
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{TDNN}}}
%& {Proposed}
%& {2.09\%} & {00.00\%} & {00.00\%} \\
%& {+FT+RA}
%& {00.00\%} & {00.00\%} & {00.00\%} \\
%\midrule
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Fast-}}}
%& {Conventional}
%& {2.16\%} & {00.00\%} & {00.00\%} \\
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ResNet}}}
%& {Proposed}
%& {3.39\%} & {00.00\%} & {00.00\%} \\
%& {+FT+RA}
%& {00.00\%} & {00.00\%} & {00.00\%} \\

\bottomrule
\end{tabular}
}
\end{center}
\end{table}
%

==> tables/table3.tex <==
\begin{table}[t] \begin{center}
%\captionsetup{singlelinecheck = false, justification=justified}
%\caption{DER on two SD benchmarks, where FT denotes the fine-tuned SE model.}
\caption{DER on two SD benchmarks.}
\resizebox{0.95\columnwidth}{!}{
\begin{tabular} {cccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{SE Model}}}&
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{SE Extraction Method}}}&
{\textbf{Extraction}}&
\multicolumn{4}{c}{\textbf{Shift size (Window size was 2.0 s)}}\\
& {\textbf{Method}}& {0.5 s} & {1.0 s} & {1.5 s} & {2.0 s} \\
%&& {0.5 s} & {1.0 s} & {1.5 s} & {2.0 s} \\
\midrule
&&\multicolumn{4}{c}{\textbf{ AMI evaluation set }}\\
\cline{3-6} \\[-1em]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ECAPA-}}}
& {Conventional}
& {17.58\%} & {18.80\%} & {20.20\%} & {21.85\%} \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{TDNN}}}
& {Proposed}
& {17.89\%} & {19.12\%} & {20.30\%} & {22.00\%} \\
& {Proposed+FT}
& {17.65\%} & {18.93\%} & {20.23\%} & {21.75\%} \\
\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Fast-}}}
& {Conventional}
&{17.75\%} & {19.12\%} & {20.33\%} & {22.03\%} \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ResNet}}}
& {Proposed}
& {18.20\%} & {19.49\%} & {20.86\%} & {22.53\%} \\
& {Proposed+FT}
& {17.79\%} & {18.99\%} & {20.28\%} & {21.60\%} \\
\midrule

%&&\multicolumn{4}{c}{\textbf{ DIHARD III test set }}\\
%\cline{3-6}
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ECAPA-}}}
%& {Conventional}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{TDNN}}}
%& {Proposed}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%& {+FT+RA}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%\midrule
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Fast-}}}
%& {Conventional}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ResNet}}}
%& {Proposed}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%& {+FT+RA}
%& {00.00\%} & {00.00\%} & {00.00\%} & {00.00\%} \\
%\midrule

&&\multicolumn{4}{c}{\textbf{ VoxConverse test set }}\\
\cline{3-6} \\[-1em]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ECAPA-}}}
& {Conventional}
& {11.82\%} & {11.98\%} & {12.60\%} & {12.98\%} \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{TDNN}}}
& {Proposed}
& {12.09\%} & {12.71\%} & {12.91\%} & {13.18\%} \\
& {Proposed+FT}
& {11.58\%} & {11.88\%} & {12.72\%} & {12.94\%} \\
\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Fast-}}}
& {Conventional}
& {12.07\%} & {12.73\%} & {12.87\%} & {13.68\%} \\
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{ResNet}}}
& {Proposed}
& {12.69\%} & {13.29\%} & {13.74\%} & {14.11\%} \\
& {Proposed+FT}
& {12.08\%} & {12.74\%} & {13.16\%} & {13.56\%} \\
\bottomrule

\end{tabular}
}
\end{center}

\end{table}
%
